Low-tubal-rank Tensor Completion using Alternating Minimization

The low-tubal-rank tensor model has been recently proposed for real-world multidimensional data. In this paper, we study the low-tubal-rank tensor completion problem, i.e., to recover a third-order tensor by observing a subset of its elements selected uniformly at random. We propose a fast iterative algorithm, called {\em Tubal-Alt-Min}, that is inspired by a similar approach for low-rank matrix completion. The unknown low-tubal-rank tensor is represented as the product of two much smaller tensors with the low-tubal-rank property being automatically incorporated, and Tubal-Alt-Min alternates between estimating those two tensors using tensor least squares minimization. First, we note that tensor least squares minimization is different from its matrix counterpart and nontrivial as the circular convolution operator of the low-tubal-rank tensor model is intertwined with the sub-sampling operator. Second, the theoretical performance guarantee is challenging since Tubal-Alt-Min is iterative and nonconvex in nature. We prove that 1) Tubal-Alt-Min guarantees exponential convergence to the global optima, and 2) for an $n \times n \times k$ tensor with tubal-rank $r \ll n$, the required sampling complexity is $O(nr^2k \log^3 n)$ and the computational complexity is $O(n^2rk^2 \log^2 n)$. Third, on both synthetic data and real-world video data, evaluation results show that compared with tensor-nuclear norm minimization (TNN-ADMM), Tubal-Alt-Min improves the recovery error dramatically (by orders of magnitude). It is estimated that Tubal-Alt-Min converges at an exponential rate $10^{-0.4423 \text{Iter}}$ where $\text{Iter}$ denotes the number of iterations, which is much faster than TNN-ADMM's $10^{-0.0332 \text{Iter}}$, and the running time can be accelerated by more than $5$ times for a $200 \times 200 \times 20$ tensor.

==> Sections/ADMM.tex <==
\section{ADMM Approach (previously used)}\label{sect:baseline}

   Based on tensor-nuclear-norm (a counterpart of matrix nuclear-norm), we formulate the following LASSO problem for noisy tensor completion:
   \begin{equation}\label{tensor_completion}
   \begin{split}
    \hat{\mathcal{T}} = \arg \min_{\mathcal{X}} &~~|| \mathcal{P}_{\Omega}(\mathcal{Y} - \mathcal{X}) ||_F^2 + \lambda || \mathcal{X} ||_{TNN}.\\
   \end{split}
   \end{equation}
   Following the ADMM framework, we introduce an intermediate variable $\mathcal{Z}$ and have:
   \begin{equation}\label{problem_admm}
    \hat{\mathcal{T}} = \arg \min_{\mathcal{X}} ~~|| \mathcal{P}_{\Omega}(\mathcal{Y} - \mathcal{X}) ||_F^2 + \lambda || \mathcal{Z} ||_{TNN}, ~~~~
    s.t. ~~\mathcal{X} = \mathcal{Z}.
   \end{equation}
   An iterative algoithm for (\ref{problem_admm}) is given in Algorithm \ref{alg:non_puncturing}.  The augmented Lagrangian of (\ref{problem_admm}) is:
   \begin{equation}
   L_{\alpha}(\mathcal{X},\mathcal{Z},\mathcal{Q}) = || \mathcal{P}_{\Omega}(\mathcal{Y} - \mathcal{X}) ||_F^2 + \lambda || \mathcal{Z} ||_{TNN}  + (\mathcal{X}(:) - \mathcal{Z}(:))^T\mathcal{Q}(:) + \frac{\alpha}{2} || \mathcal{X} - \mathcal{Z}||_F^2,
   \end{equation}
   and the corresponding recursion steps are:
  \begin{eqnarray}
%   %\begin{split}
   \mathcal{X}^{k+1} &&= \arg~\min\limits_{\mathcal{X}}~ || \mathcal{P}_{\Omega}(\mathcal{Y} - \mathcal{X}) ||_F^2  + (\mathcal{X}(:) - \mathcal{Z}^k(:))^T\mathcal{Q}^k(:) + \frac{\alpha}{2} || \mathcal{X} - \mathcal{Z}^k||_F^2, \\
   \mathcal{Z}^{k+1} &&= \arg~\min\limits_{\mathcal{Z}}~ \lambda || \mathcal{Z} ||_{TNN}  + (\mathcal{X}^{k+1}(:) - \mathcal{Z}(:))^T\mathcal{Q}^k(:) + \frac{\alpha}{2} || \mathcal{X}^{k+1} - \mathcal{Z}||_F^2,\\
   \mathcal{Q}^{k+1} &&= \mathcal{Q}^k + \alpha (\mathcal{X}^{k+1} - \mathcal{Z}^{k+1}),
%   %\end{split}
   \end{eqnarray}
   where $\alpha$ and $\mathcal{Q}$ are multipliers, $\mathcal{X}(:)$ and $\mathcal{Q}(:)$ means vectorizing the tensors (it is MATLAB notation).

   The solution for $\mathcal{X}^{k+1}$ is given by
   $\mathcal{X}^{k+1} = (\alpha \mathcal{I} + \mathcal{P}_{\Omega})^{-1} (\mathcal{Y} + \alpha (\mathcal{Z}^{k} - \mathcal{Q}^{k}))$,
   where $\mathcal{I}$ is the identity tensor. It is essentially a closed-form solution to the least squares problem. Let $\mathcal{P}_{\Omega'} = (\alpha \mathcal{I} + \mathcal{P}_{\Omega})^{-1}$, $I\in \mathbb{R}^{N_1 \times N_2}$ be a matrix with $I(i,i)=1$ and $I(i,j)=1$ for $i \neq j$, where $\Omega, \Omega'$ are indicator matrices.
   Note that $\Omega$ in Subsection \ref{problem_statement} is binary, and the $(i,j,k)$-th entry of $\mathcal{P}_{\Omega}(\mathcal{X})$ is equal to $\mathcal{X}(i,j,k)$ if $(i,j)\in \Omega$ and zero otherwise.
   $\Omega'$ can be calculated as follows: for the diagonal elements, $\Omega'(i,i)=\frac{1}{\alpha I(i,i) + \Omega(i,i)}$, and for the non-diagonal elements, $\Omega'(i,j)= 1$ if $\Omega(i,j) =0$ and $\Omega'(i,j)= 0$ if $\Omega(i,j) =1$, $\forall i \neq j$. Then, $\mathcal{X}^{k+1} = \mathcal{P}_{\Omega'} (\mathcal{Y} + \alpha (\mathcal{Z}^{k} - \mathcal{Q}^{k}))$ is calculated by scaling the $(i,j)$-th tube of $(\mathcal{Y} + \alpha (\mathcal{Z}^{k} - \mathcal{Q}^{k}))$ by a factor $\Omega'(i,j)$.

   The solution for $\mathcal{Z}^{k+1}$ is given by:
   \begin{equation}\label{update_step_Z}
   \mathcal{Z}^{k+1} = \arg~\min\limits_{\mathcal{Z}}~ \frac{\lambda}{\alpha} || \mathcal{Z} ||_{TNN}  + \frac{1}{2} || \mathcal{Z} - (\mathcal{X}^{k+1} + \frac{1}{\alpha}\mathcal{Q}^{k}) ||_F^2,
   \end{equation}
   where scaling the objective value by $1/\alpha$ does not change the optimal solution.
   Let $A = U \Sigma V$ be the singular value decomposition of matrix $A$. We define the singular value thresholding operator as
   $\mathcal{D}_{\epsilon}(A)= U \mathcal{S}_{\epsilon}[\Sigma] V$,
   where $\mathcal{S}[\cdot]$ is an element-wise thresholding operator,
   i.e., $\mathcal{S}_{\epsilon}[x] = x - \epsilon,~\text{if}~x > \epsilon$, $\mathcal{S}_{\epsilon}[x] = x + \epsilon,~\text{if}~x < -\epsilon$, and $\mathcal{S}_{\epsilon}[x] = 0$, otherwise.

  Therefore, the optimal solution to (\ref{update_step_Z}) is:
  \begin{equation}
  \text{blkdiag}(\breve{\mathcal{Z}}) = \mathcal{D}_{\frac{\lambda}{\alpha}}(\text{blkdiag}(\text{fft}(\mathcal{X}^{k+1} + \frac{1}{\alpha}\mathcal{Q}^k),[~],3)),
  \end{equation}
  which thresholds the eigenvalues of the block diagonal matrix  $\text{blkdiag}(\text{fft}(\mathcal{X}^{k+1} + \mathcal{Q}^k),[~],3)$ by $\frac{\lambda}{\alpha}$.

  %The detailed algorithm is shown in Algorithm \ref{alg:non_puncturing}.
  For algorithm implementation, one can initialize $\mathcal{Z}^0$ and $\mathcal{Q}^0$ as zero tensors. $\Omega$ is an indicator matrix of size $N_1 \times N_2$, i.e., $\Omega_{ij}=1$ with probability $\frac{M}{N_1N_2}$.
  The iteration criteria for {\em not converged} is: the change of the objective value $L_{\alpha}(\mathcal{X},\mathcal{Z},\mathcal{Q})$ during two consecutive iterations is larger than a preset threshold, and $k$ is less than a preset number of maximum iterations. %As a direct consequence of \cite{Shuchin2015PAMI} and \cite{Candes2010}, we have the following performance guarantee.

\begin{algorithm}[h]
  \caption{ADMM Algorithm}
  \label{alg:non_puncturing}
  \begin{algorithmic}
  \STATE \textbf{Input}: $\mathcal{P}_{\Omega}(\mathcal{T}), \Omega, \lambda,\alpha$
  \STATE $\mathcal{Z}^0 \leftarrow 0; \mathcal{Q}^0 \leftarrow 0; k \leftarrow 0$.
  %\STATE $\Omega \leftarrow \text{mask}(N_1,N_2,M)$;
  \WHILE{not converged}
       \STATE $ \mathcal{X}^{k+1} \leftarrow (\alpha \mathcal{I} + \mathcal{P}_{\Omega})^{-1} (\mathcal{Y} + \alpha(\mathcal{Z}^{k} - \mathcal{Q}^{k}))$.
       \STATE $\text{blkdiag}(\breve{\mathcal{Z}}) \leftarrow \mathcal{D}_{\frac{\lambda}{\alpha}}(\text{blkdiag}(\text{fft}(\mathcal{X}^{k+1} + \frac{1}{\alpha}\mathcal{Q}^k),[~],3))$, and obtain $\breve{\mathcal{Z}}$ from $\text{blkdiag}(\breve{\mathcal{Z}})$.
       \STATE $\mathcal{Q}^{k+1} \leftarrow  \mathcal{Q}^k + \alpha (\mathcal{X}^{k+1} - \mathcal{Z}^{k+1})$; ~$k \leftarrow k+1$.\\
  \ENDWHILE
  \end{algorithmic}
  \vspace{-2pt}
\end{algorithm}



==> Sections/Codes.tex <==
\section{Codes}

  Following the notations in ``Notes on Random Sampling" (Josh Girson)

  \begin{equation}
  \hat{\mathcal{X}} = \argmin_{\hat{\mathcal{X}} \in \mathbb{R}^{n \times r \times k}} ||\hat{\mathcal{T}}_{\Omega} - \hat{\mathcal{P}}_{\Omega} \cdot\otimes (\hat{\mathcal{X}}~\cdot\S~ \hat{\mathcal{Y}}) ||_F^2,
  \end{equation}
  where $\cdot \otimes$ denotes tube-wise circular convolution, $\cdot \S$ denotes front-slice-wise matrix multiplication.

  \begin{equation}\label{LS_equal}
  \hat{\mathcal{X}}^T = \argmin_{\hat{\mathcal{X}}^T \in \mathbb{R}^{r \times n \times k}} ||\hat{\mathcal{T}}_{\Omega}^T - \hat{\mathcal{P}}_{\Omega}^T \cdot\otimes (\hat{\mathcal{Y}}^T ~\cdot\S~  \hat{\mathcal{X}}^T ) ||_F^2,
  \end{equation}
  where $\mathcal{X}^T$ denotes the tube-wise transpose (the transpose of a matrix  by regarding $\mathcal{X}^T$ as a matrix of vectors).

  The problem (\ref{LS_equal}) estimates $\hat{\mathcal{X}}^T$, which can be decomposed into $m$ separate least squares problem. In other words, each lateral slice of $\hat{\mathcal{X}}^T$ can be estimated separately.

  Note that: as $\cdot \otimes$ is tube-wise circular convolution, such decomposition is OK. While estimating each lateral slice, we can further transform $\cdot \otimes$ into matrix operations.


==> Sections/RelatedWork.tex <==
\section{Related Work}

   There are two major differences between existing works and our work:
   \begin{itemize}
     \item Several recent works [x] show that for matrix completion, alternating minimization xxx. Such results cannot be directly applied to the tensor case. (why not?)
     \item For other tensor model, such an algorithm has been proposed [x]. No performance guarantees are provided.
   \end{itemize}


    1. Algorithms for low-order tensors

     why the techniques in matrix completion and low CP-rank tensor completion cannot be extended to deal with our case in a straightforward way? We need high level explanations.

    2. Algorithms for high-order tensor without performance guarantee.


==> Sections/Related_works.tex <==
\section{Background and Existing Works}

   In this section, we first introduce the execution flow and framework of fingerprint-based localization and then summarize existing schemes.
   %At last, we survey and compare with existing results for low-rank matrix/tensor completion.

\subsection{Overview of Fingerprint-based Localization}

%  In the site survey phase, there are two generally adopted approaches for sampling the reference points: (1) full-map sampling. Divide the region of interest into a grid map (e.g., grid size $1$ m $\times$ $1$ m), then sample all the reference points that lies on the grid map. (2) Partial-map sampling. The system builders selectively sample some points within the area of interest without considerations for the operating phase. The fingerprinting database just stores the RSS fingerprints at the sampling locations.

\subsection{Existing Works}

  %As mentioned in Section I, there are three approaches for indoor localization. In this section, we concentrates on existing schemes that fall within fingerprint-based approach and those aiming at reliefing the burden of site survey.
  In this section, we first describe exemplar systems for fingerprint-based approach and then survey recently proposed schemes.

  Fingerprint-based localization systems can be classified into the following three categories: RF fingerprint-based, non-RF fingerprint-based, and cross-technology-based. RADAR \cite{RADAR2000} and Google Indoor Map \cite{GoogleMap} utilize RF fingerprint; IndoorAtlas \cite{IndoorAtlas} utilizes the magnetic field map as fingerprint; and SurroundSense \cite{Azizyan2009MobiCom} and WiFiSLAM \cite{WiFiSLAM} are cross-technology-based. RADAR \cite{RADAR2000} is considered as the first fingerprint-based system, even one of the first indoor localization systems. SurroundSense \cite{Azizyan2009MobiCom} exploits ambient attributes (sound, light, etc) including RF fingerprint. Google Indoor Map \cite{GoogleMap} and WiFiSLAM \cite{WiFiSLAM} are two widely used industrial apps on smartphones, while the former one uses RF fingerprints that are directly sampled and stored, the later one incorporates user trajectories, inertial information and accelerometer.

  The major challenge for indoor localization systems lies in the time- and manpower-consuming site survey process. Recently, there are many works aiming to relieve this burden, which we broadly classify into correlation-aware approach, crowdsourcing-based approach, and sparsity-aware approach.

  The correlation-aware approach leverages the key observation that the fingerprints at nearby reference points are spatially correlated. For example, \cite{Li2005IEE} utilized the kriging interpolation method while \cite{Kuo2011TMC} adopted the kernel functions (continuous and differentiable discriminant functions) and proposed discriminant minimization search. Such schemes try to use linear or non-linear functions to model the correlations, which are essentially model-based approaches and face similar limiting factors as discussed in the Introduction.

  It seems attractive to remove the off-line site survey and instead incorporating users' online cooperation, which is the basic idea of {\em crowdsourcing}-based approach. For example, LiFS \cite{Yang2012MobiCom} leveraged reported user trajectories (RF fingerprints and step counts) to establish a one-to-one mapping between RF fingerprints and the digital flor plan map. Note that digital map is not always available. Jigsaw \cite{Jigsaw2014MobiCom} exploited image processing techniques to reconstruct flor plans based on crowdsourcing collected pictures. Zee \cite{Rai2012MobiCom} was another crowdsourcing-based scheme that leveraged the inertial sensors (e.g., accelerometer, compass, gyroscope) to track users as they traverse an indoor environment while simultaneously performing WiFi scans. However, the crowdsourcing-based approach is fundamentally the application of machine learning on large-scale data sets thus requires a large number of users to report to the server, and even more, it incurs high energy comsumption on smartphones.

  A promising approach is to apply the emerging compressive sensing tool that models the spatial correlation as sparse (or low-rank). \cite{Zhang2013WCNC} assumed that the RSS matrix for each access point was low-rank and \cite{Hu2013} further assumed that the low-rank matrix was smooth; but both failed to exploit the cross correlations among the access points. \cite{Milioris2014} more generally asserted that the fingerprint data is low-dimensional, however, uniform sampling is adopted. Different from the above mentioned schemes, we propose to employ adaptive sampling for the sake of cutting down the sampling burden.

  Note that some existing works adopted compressive sensing by exploiting other forms of sparsity. For example, since the number of candidate locations for a query fingerprint is relatively small compared to the size of the whole grip map, \cite{Feng2012TMC} proposed a two-phase localization algorithm based on $\ell_1$ minimization; and the number of changes in the fingerprint data for two consecutive period is relatively small compred to the size of the whole grid map, \cite{Zhu2014} dealt with the updating process for the localization system.
  Although these schemes exploit sparsity, they differ fundamentally from our proposed approach.

  %As smartphones are set to automatically sample along users' trajectories, RSS fingerprints\footnote{Note that there is no location information associated with each fingerprint of LiFS, which is different from traditional fingerprint-based approach.} are geographically connected, while the physical distances among fingerprints are reflected by footsteps. Therefore, human motions can be applied to connect RSS fingerprints. Motivated by this observation, the authors of \cite{Yang2012MobiCom} propose to use digital maps as {\em a prior} information to locate the fingerprints.



  %In the cell-based approach \cite{Zhao2002}\cite{Voronois2003}\cite{Barabasi2005}, each user's location is given by the access point (with known coordinates, called {\em anchors}) to which it is connected. Therefore, the localization error is essentially determined by the communication range and the distances between the access points. In indoor environment, the cell-based approach captures room-level location information as AP deployers tend to put one AP in each room and thus its localization error is usually on the order of $10$m $\sim$ $20$m.
  %A number of model-based schemes \cite{Poor2005SPG}\cite{Gustafsson2005SPG}\cite{Win2011} have been proposed based on some physical quantities to measure distances from signal sources (anchors), such as angle of arrival (AoA), time of arrival (ToA), time difference of arrival (TDoA), and received signal strength (RSS). These schemes estimate locations based on geometrical models, such as trilateration, multilateration, and triangulation. The prevalent log-distance path loss model, for instance, builds up a semi-statistical function between RSS values and radio propagation distances. Most existing schemes report median localization errors of $2$m $\sim$ $8$m. The key to further improve localization accuracy is to establish more accurate models for the fading effects of signal propagations. However, in indoor environment, this is essentially prohibited by the following factors: 1) low transmission power, 2) high attenuation caused by walls and furnitures, 3) complicated surface reflections, and 4) unpredicted dynamics, e.g., disturbance caused by human movements.

  %The fingerprint-based approach attracts many research efforts recently. It is a two-phase approach, a training phase and an operating phase. In the training phase, a fingerprinting database of an area of interest is built up {\em a prior} for localization. In the operating phase, the location estimation is then to match the query fingerprint with candidate locations in the fingerprint database. The advantages are, 1) it is a passive approach that does not need the locations of APs, i.e., using WiFi APs which already deployed in most buildings thus circumventing extra infrastructure deployment, 2) RSS interface is already provided by off-the-shelf WiFi- or Zigbee-compatible devices, 3) the flourish of smartphone market indicates its potential wide use, and 4) there is no assumed model and thus the approach is resilient to whether a particular path loss model holds. Most of these techniques utilize the ambient radio signals such as RADAR \cite{RADAR2000}, Horus \cite{Youssef2005} (improved upon RADAR), LANDMARC \cite{LANDARC}, and ActiveCampus \cite{ActiveCampus}. SurroundSense \cite{Azizyan2009MobiCom} performs logical location estimation based on ambient features including sound, light, color, WiFi, etc. Those schemes report median localization errors of $2$ m $\sim$ $8$ m, similar as the model-based approach. However, all fingerprint-based methods require a site survey process to build a fingerprint database. The considerable manual costs and efforts of site survey, in addition to the inflexibility to environment dynamics are the main drawbacks. For example, in the end of 2011, Google released Google Map 6.0 that provides indoor localization and navigation available only at some selected airports and shopping malls in the US and Japan. The enlargement of applicable areas is strangled by pretty limited fingerprint data of building interiors. In this paper, we propose a new way of localizing in indoor environments where good location estimates can be achieved with a limited number of measurements.

  %We briefly describe three representative systems, RADAR \cite{RADAR2000}, SurroundSense \cite{Azizyan2009MobiCom}, and LiFS \cite{Yang2012MobiCom}. The pioneer indoor localization system, RADAR \cite{RADAR2000}, passively collects WiFi RSS at many positions and orientations throughout a building. On the previously built data set, the localization estimation is simply obtained by performing table lookup. The Euclidean distance is adopted as a dissimilarity metric and a KNN (i.e., {\em nearest neighbor(s) in signal space (NNSS)}) technique is applied to compare multiple locations and then picks the one that best matches the observed RSS vector. Besides WiFi RSS, SurroundSense \cite{Azizyan2009MobiCom} uses multiple physical attributes (ambient sound, light, color, and human movement) as fingerprints. It is shown that such a logical fingerprint space is identifiable and multi-mode fingerprints can collaborate to provide better localization performance. LiFS \cite{Yang2012MobiCom} is the first trial to reduce the burden of site survey, while a {\em crowdsourcing}-based approach is proposed to replace the {\em delicately-controlled} site survey process. As smartphones are set to automatically sample along users' trajectories, RSS fingerprints\footnote{Note that there is no location information associated with each fingerprint of LiFS, which is different from traditional fingerprint-based approach.} are geographically connected, while he physical distances among fingerprints are measured by footsteps. Therefore, human motions can be applied to connect RSS fingerprints. Motivated by this observation, the authors of \cite{Yang2012MobiCom} propose to use digital maps as {\em a prior} information to locate the fingerprints.


==> Sections/Simulation.tex <==
\section{Simulation Results}

 % In this section, we conduct extensive simulations to test the locality of the fingerprint space, the recovery performance of our puncturing approach, and the localization performance of stardard localization schemes over the rebuilt fingerprint space.

\subsection{Experiment Setup}

  \begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{pic/Scenario.eps}
  \includegraphics[width=0.26\textwidth]{pic/Colorbar.eps}
  \caption{We select a rectangle area within an office building for simulations. RSS is measured in dBm.}\label{fig:scenario}
  \end{figure}

  %\textbf{Ground truth}:

  We select a region of $47.5$m $\times$ $59.7$m in a real office building, as shown in Fig. \ref{fig:scenario}. It is divided into a $476 \times 598$ grid map. There are $15$ access points randomly deployed within this region.
  The indoor radio channel is characterized by multi-path propagation with dominant propagation phenomena: the shadowing of walls, wave guiding effects in corridors due to multiple reflections, and diffractions around vertical wedges.
  The ray tracing model \cite{SRT,Ray_tracing_TWC2009} is adopted, which considers all these effects leading to highly accurate prediction results.
  We generated a $476 \times 598 \times 15$ RSS tensor as the {\em ground truth} for our simulations. Note that the RSS values are measured in dBm. For example, the RSS radio map for the $5$-th and $15$-th access points are shown in Fig. \ref{fig:rss-map}.

  \begin{figure}[t]
  \centering
  \includegraphics[width=0.49\textwidth]{pic/RSS_map_5th.eps}
  \includegraphics[width=0.49\textwidth]{pic/RSS_map_15th.eps}
  \caption{The RSS radio map of the $5$-th and $15$-th access points.}\label{fig:rss-map}
  \end{figure}

  We are interested in two kinds of performance: recovery error and localization error. Varying the sampling rate as $10\% \sim 90\%$, we quantify the recovery error in terms of {\em normalized square of error (NSE)} for entries that are not sampled, i.e., recovery error for set $\Omega^{c}$. The NSE is defined as:
  \begin{equation}
  NSE = \frac{\sum_{(i,j)\in \Omega^{c}} ||\hat{\mathcal{T}}(i,j,:) - \mathcal{T}(i,j,:) ||_F^2 }{ \sum_{(i,j)\in \Omega^{c}} ||\mathcal{T}(i,j,:)||_F^2 },
  \end{equation}
  where $\hat{\mathcal{T}}$ is the estimated tensor, $\Omega^{c}$ is the complement of set $\Omega$.

  In the simulations, we uniformly select $500$ testing points within the selected region and then using the classic localization schemes to perform localization estimation. We measure the localization error as the Euclidean distance between the estimated location and the actual location of the testing point, i.e.,
  $d_e = \sqrt{(\hat{x}_1 - x_1)^2 + (\hat{x}_2 - x_2)^2}$.

%  We further define a {\em failure rate} as the faction of testing points that has distance error bigger than $1$m since we care about sub-meter localization. It is defined as:
%  \begin{equation}
%  \text{FR} = \sum_{i=1}^{N}\mathbb{I}_i(d_e^i > 1) / N,%,~~\text{FR-II} = \mathbb{I}(d_e > 2) / N,
%  \end{equation}
%  where $N$ is the number of testing points, and $d_e^i$ is the error distance of the $i$-th testing point. In the simulations, we uniformly select $500$ testing points within the selected region and then using the classic localization schemes to perform localization estimation.

%\subsection{Locality Verification}
%
%  \begin{figure}[t]
%  \centering
%  \includegraphics[width=0.60\textwidth]{pic/locality_verification.eps}
%  \caption{The locality of the fingerprint space with KNN, Kernel approach and SVM under three cases: without noise, $3$ dBm and $10$ dBm noise cases.}\label{fig:locality}
%  \end{figure}
%
%  Fundamentally, it is important to know the locality of the fingerprint space, namely, if we have the ground truth already, what kind of localization performance can we expect to achieve by KNN, Kernel approach, and SVM. The locality of the fingerprint space directly determines the localization ability of any fingerprint-based scheme. It strongly relates to the difference between the fingerprint vectors at nearby points. If the fingerprints differ from each other substantially, then the fingerprint space has strong locality, otherwise, the fingerprint space has weak locality.
%
%  Another important factor is the measurement noise in the fingerprint database. The noise may come from collection error or the dynamics in the environment. If the measurement process has high SNR, say $3$ dBm, then we can expect the localization results to achieve the best performance of the fingerprint space, i.e., the locality of the fingerprint space. If the measurement process has low SNR, say $10$ dBm, then we still hope to obtain acceptable localization performance. Therefore, we test three cases for locality verification: without noise, high SNR, and low SNR.
%
%  Fig. \ref{fig:locality} shows the results of our locality verification. If there is no noise in the inquiry fingerprint, both KNN and Kernel approach can achieve almost zero error (less than $10^{-3}$ m). All testing points has localization error less than $0.05$ m, while $90\%$  are almost zero. For $3$ dBm noise (high SNR), all three localization schemes has localization error less than $0.05$ m, and less than $0.5$ m for $10$ dBm noise (low SNR). Note that it is $0.2$ m for SVM. Therefore, we see that the fingerprint space has really strong locality and it has the potential to achieve our goal of sub-meter indoor localization.

\subsection{Radio Map Recovery Performance}\label{sect:recovery}

%  \begin{figure}[t]
%  \centering
%  \includegraphics[width=0.49\textwidth]{pic/Recovery_error_TC.eps}
%  \caption{The recovery error of tensor completion under uniform sampling and puncturing for different sampling rates.}\label{fig:tc_recovery}
%  \end{figure}

  For comparison, we adopt two algorithms, tensor completion via uniform tubal-sampling \cite{Shuchin}, % (as described in Section \ref{sect:baseline}),
  and matrix completion via uniform sampling \cite{Kong2013INFOCOM}. The alternative direction algorithm \cite{Kong2013INFOCOM} is much faster than the singular value thresholding algorithm \cite{Candes2010SIAM,Candes2010,Recht2010,MC_noise}. To recover the RSS tensor, matrix completion estimates each RSS matrix separately and independently.
  %Note that we do not use matrix completion via adaptive sampling \cite{Singh2013NIPS} because for fingerprinting calibration the engineer samples a RSS vector at each reference point which is vector-wise sampling, and the entry-wise sampling would turn out to be rather inefficient.


%  We test the recovery performance of matrix completion under puncturing method and uniform sampling. We vary the sampling rate (i.e, the sampling budget) as $10\%$, $20\%$, ..., $90\%$. For uniform sampling, the samples are uniformly distributed across the selected area. It serves as a baseline for our puncturing method.


  Fig. \ref{fig:recovery} shows the RSS tensor recovery performance for varying sampling rate. Compared schemes are matrix completion and tensor completion via uniform sampling, and adaptive sampling with allocation ratio $\delta = 1/4$ and $\delta = 1/2$. We find that all tensor approaches are better than matrix completion, this is because tensor exploits the cross correlations among access points while matrix completion only takes advantage of correlation within each access point. Both AS schemes outperform tensor completion via uniform sampling since adaptivity can guide the sampling process to concentrate on more informative entries. Allocating equal sampling budget for the $1$st-pass and the $2$nd-pass gives better performance than uneven allocation. This shows that the $1$st-pass and the $2$nd-pass have equal importance. The proposed scheme (AS with $\delta = 1/2$) rebuilds a fingerprint data with $5\%$ error using less than $30\%$ samples. %, i.e., the adaptive puncturing scheme reduces the sampling budget by $70\%$.

%   Fig. \ref{fig:recovery} shows the NSE error of matrix completion. Two important parameters in our puncturing scheme is the allocation ratio $\delta$ and the distillation ratio $\gamma$. Set $\delta = 1/2$ generally has lower recovery error than that of $\delta = 1/4$. This means that if allocate more samples to concentrate on the strong blocks (area regions with stronger RSS), we can generally build a more accurate fingerprint space and thus expect to have better localization performance. Moreover, smaller distillation ratio ($\gamma = 0.7$) benefits more the recovery accuracy than bigger distillation ratio ($\gamma = 0.9$). Cases with smaller $\gamma$ have equal results with cases of smaller $\delta$, both leads to concentrating the samples to the strong blocks. However, too clustered samples will lead to bad recovery since we lose information of many blocks.
%
%   Fig. \ref{fig:recovery}(b) shows the NSE error of tensor completion. Compared with matrix completion, tensor completion has lower recovery error. The reasons are (1) tensor completion exploits the inter-correlations between the RSS matrices of all APs, i.e., the propagation of radio frequency signals follow the same principle.

%  \begin{figure}[t]
%  \subfigure[Matrix Completion]{\includegraphics[width=0.5\textwidth]{pic/Recovery_error_MC.eps}}
%  \subfigure[Tensor Completion]{\includegraphics[width=0.5\textwidth]{pic/Recovery_error_TC.eps}}
%  \caption{The recovery error of matrix completion and tensor compeletion under uniform sampling and puncturing for different sampling settings.}\label{fig:recovery}
%  \end{figure}

  \begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{pic/AP_Comparison.eps}
  \caption{Tensor recovery for varying sampling rate. MC denotes matrix completion via uniform sampling, TC denotes tensor completion via uniform sampling, while AS-$1/4$ and AS-$1/2$ denote our adaptive sampling scheme with allocation ratios $\delta = 1/4$ and $\delta = 1/2$, respectively.}\label{fig:recovery}
  \end{figure}

\subsection{Localization Performance}

  An important factor that influences the localization error is the measurement noise. Note that for site survey, the engineer stays for a while to obtain a stable fingerprint. Therefore, we only consider measurement noise in the query fingerprint. The noise may come from the measuring process or the dynamics in the environment. High SNR and low SNR cases are considered. For the high SNR case we add $3$dBm Gaussian noise, while $10$dBm Gaussian noise is added for the low SNR case.

  We choose three representative localization techniques for comparison, namely, weighted KNN, the kernel approach, and support vector machine (SVM).
  KNN (weighted KNN) is the most widely used technique since it is simple and is reported to have good performance in indoor localization systems \cite{RADAR2000}\cite{Yang2012MobiCom}. The kernel approach is an improved scheme over weighted KNN, which can be regarded as the basic principle of all machine learning-based localization approaches. The kernel function encapsulates the complicated relationship between RF fingerprints and physical positions. SVM is an efficient machine learning method widely used in fingerprint-based indoor localization. SVM uses kernel functions and tries to learn the complicated relationship between RF fingerprints and physical positions by regression.

  In addition to localization based on the estimated tensor $\hat{\mathcal{T}}$, we also test the above three localization techniques on the samples $\mathcal{Y}$ (without doing any reconstruction or estimation). Let DL denote {\em direct localization (DL} on uniformly sampled fingerprints, while DL-$1/4$ and DL-$1/2$ denote direct localization on adaptively sampled fingerprints with allocation ratios $\delta = 1/4$ and $\delta = 1/2$, respectively.

  %\textbf{1. (Weighted) KNN}:
\subsubsection{Weighted KNN}

\begin{figure}[t]
\subfigure{\includegraphics[width=0.49\textwidth]{pic/KNN_3dBm.eps}}
\subfigure{\includegraphics[width=0.49\textwidth]{pic/KNN_10dBm.eps}}
\caption{The empirical CDFs of localization error of KNN with $20\%$ samples for $3$dBm noise case and $10$dBm noise case. MC denotes matrix completion via uniform sampling, TC denotes tensor completion via uniform sampling, DL denotes direct localization on uniformly sampled fingerprints, while AS denotes our adaptive sampling scheme. For adaptive DL and AS, there are two allocation ratios $\delta = 1/4$ and $\delta = 1/2$.}\label{fig:KNN}
\end{figure}

%\begin{figure}[t]
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/final_40percent_knn_noise.eps}}
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/ft_40percent_knn_noise.eps}}
%\caption{The empirical CDF of localization error and failure rate of KNN with $40\%$ samples, $10$ dBm noise.  The same legend with Fig. \ref{fig:knn_40percent}.} \label{fig:knn_40percent_noise}
%\end{figure}

  Let $k$ be a fixed positive integer which are usually set to be $1,3,5,7,$ etc., consider a sampled fingerprint $r_p$ at reference point $p$. Find within the fingerprint database $\mathcal{F}$ the reference point locations $p_1,p_2,...,p_k$ whose fingerprints are nearest to $r_p$. Then, estimate the location $p$ by weighted averaging $p_1,p_2,...,p_k$ as follows:
   \begin{equation}\label{knn_form}
   \hat{p} = %\frac{\sum_{i=1}^{k} \frac{p_i}{d(r_{p_i},r_p) + d_0} }{\sum_{i=1}^{k} \frac{1}{d(r_{p_i},r_p) + d_0}} =
   \sum_{i=1}^{k}p_i~ \frac{ \frac{1}{d(r_{p_i},r_p) + d_0} }{\sum_{i=1}^{k} \frac{1}{d(r_{p_i},r_p) + d_0}},
   \end{equation}
   where $d(r_{p_i},r_p)$ is the Euclidean distance between the two fingerprints, and $d_0$ is a small real constant used to avoid division by zero. In the simulations, we find that $k=5$ and $d_0 = 0.01$dBm are the best since the reference points in our experiments are located on a grid map with each reference point having $4$ neighbors (plus itself leads to $k=5$). Note that we estimate the x-coordinate and y-coordinate separately.

   Fig. \ref{fig:KNN} shows the empirical CDFs of localization error of weighted KNN with $20\%$ samples for $3$ dBm noise and $10$ dBm noise. Besides the recovery schemes compared in Section \ref{sect:recovery}, we also consider direct localization (DL) with samples drawn uniformly from the grid map and those output by the adaptive sampling approach. We find that the proposed adaptive sampling approach (both $\delta = 1/4$ and $\delta = 1/2$) dramatically outperforms other schemes. In the high SNR case, $97\%$ ($90\%$ respectively) of the reference points can be localized with error less than $2$m ($1$m), while $90\%$ ($95\%$ respectively) in the low SNR case. Such performance improvements may be explained by the performance of direct localization (uniform, adaptive with $\delta = 1/4$ and $\delta = 1/2$). Since in both high and low SNR cases, adaptive sampled RF fingerprints are more useful for localization than non-adaptive sampled RF fingerprints. To some extent, it shows that our adaptive sampling approach has identified entries that are highly informative.

   %\textbf{2. Kernel Approach}:
\subsubsection{Kernel Approach}
\begin{figure}[t]
\subfigure{\includegraphics[width=0.5\textwidth]{pic/Kernel_3dBm.eps}}
\subfigure{\includegraphics[width=0.5\textwidth]{pic/Kernel_10dBm.eps}}
\caption{The empirical CDFs for the kernel approach with the same legend as Fig. \ref{fig:KNN}.}\label{fig:kernel}
\end{figure}

   We estimate the coordinates as $\hat{p}  = \sum_{i \in H(p)} \phi(r_{p_i}, r_p) p_i + \alpha_0$,
   where $H(p)$ denotes the set of reference points whose fingerprints have the smallest Euclidean distances to the query fingerrpint, $\phi(\cdot)$ is the kernel function which can be polynomial functions, Gaussian functions, and exponential functions. In the simulations, we set $\phi(\cdot)$ to be the square distance, the cardinality of $H(p)$ be $50$. Therefore, we have:
   \begin{equation}\label{kernel_location}
   \hat{p}  = \sum_{i \in H(p)} p_i \frac{ \frac{1}{d^2(r_{p_i},r_p) + d_0^2} }{\sum_{i=1}^{k} \frac{1}{d^2(r_{p_i},r_p) + d_0^2}}.
   \end{equation}
   We can see the strong similarity with the weighted KNN. A major difference is that the number of reference points used by the kernel method is much larger than the number of neighboring reference points used by weighted KNN.

   Fig. \ref{fig:kernel} shows the empirical CDFs of localization error of the kernel approach with $20\%$ samples for $3$dBm and $10$dBm noise. Similar to KNN, the proposed scheme outperforms all other schemes. There are two interesting things to notice. First, for the kernel approach, $38\%$ testing points has zero error for adaptive sampling with $\delta = 1/2$ and $3$dBm noise. Second, compared with Fig. \ref{fig:KNN}, the kernel approach is more robust to noise. Surprisingly, the kernel approach performs better in the $10$dBm noise case than in the $3$dBm noise case. The reason is that with lower SNR, the kernel function captures the location centroid of WiFi access points, i.e., the coordinates of access points. Because (\ref{kernel_location}) is dominant by nearby (relative to the user's location) access points, and with $50$ ($|H(p)|=50$) reference points rather than $k=5$ reference points, (\ref{kernel_location}) essentially captures the location of the dominating access points \cite{Kuo2011TMC}.

\subsubsection{SVM Approach}

   %\textbf{3. SVM}:
   Support vector machines (SVM) separate reference points using linear hyperplanes in the fingerprint space. The x-coordinate and y-coordinate are estimated separately.
   Let $(x_j,y_j)$ denote the coordinates of reference point $p_j$ and $r_{p_j}$ denote the fingerprint. For $x_j$, the training data $\{(x_j, y_j),r_{p_j}\}$ become labeled-pairs $\{\Delta_i,r_{p_i}\}$ where the input is $r_{p_i}$, and the output is $\Delta_i =1$ if $x_i = x_j $ and $\Delta_i =-1$ if $x_i \neq x_j $.
   SVM construct a classifier of the form $\Delta_i(r_{p_i}) = \text{sign}[\sum_{i=1}^{N_1N_2} w_i \Delta_i \phi(r_{p_i},r_{p_j}) + b]$, where $w_i$ are positive real constants and $b$ is a real constant. The kernel function $\phi(\cdot,\cdot)$ typically has the following choices: $\phi(r_{p_i},r_{p_j}) = r_{p_i}^T r_{p_j}$ (linear SVM); $\phi(r_{p_i},r_{p_j}) = (r_{p_i}^T r_{p_j} + 1)^d$ (polynomial SVM of degree $d$); $\phi(r_{p_i},r_{p_j}) = \exp\{ - ||r_{p_i} - r_{p_j}||_2^2 /\sigma^2\}$ (radius basis function kernel SVM); $\phi(r_{p_i},r_{p_j}) = \tanh[\kappa r_{p_i}^T r_{p_j} + \theta]$ (two-layer neural SVM), where $\sigma, \kappa, \theta$ are constants. We use linear SVM in the experiments, and according to the structural risk minimization principle \cite{SVM}, we seek the solution of the following optimization problem:
   \begin{equation}
   \min_{w,b,\xi} ~\frac{1}{2}||w||_2 + C \sum_{i=1}^{N} \xi_i~~~~~\\
   s.t.~~\left\{
   \begin{aligned}
   w^T \cdot r_{p_i} + b &\geq 1 - \xi_i,~~\text{if}~~x_j = x_i, \\
   w^T \cdot r_{p_i} + b &\leq-1 + \xi_i,~~\text{if}~~x_j \neq x_i,\\
   \xi_i &~> 0.~~\\
   \end{aligned}
   \right.
   \end{equation}
   where $C$ is the penalty parameter of the error term and $\xi_i$ are introduced in case a separating hyperplane in this higher dimensional space does not exist. We use the SVM library \cite{Lib_svm}.

%   and minimize the empirical risk $R_{emp} = \frac{1}{n}\sum_{i=1}^{n} \ell(\phi(p_i), r_{p_i}) $, where $\ell(\cdot)$ is a loss function, $\ell(y,y') =1$, if $||y - y'||_2 \geq \varepsilon$ for some pre-set $\varepsilon$, and $0$ otherwise. One can use linear, Gaussian, or exponential functions as the classifier function.


%   estimate a function $r_p = \phi(p)$ from a set of training data $\{(p,r_p)\}$. %We assume the existence of a linear function $f(p) = w \cdot p + b$ in our simulation.
%   The training phase corresponds to the following optimization problem:
%   \begin{equation}
%   \min_{w} ~\frac{1}{2}||w||_2 ~~~\\
%   s.t.~\left\{
%   \begin{aligned}
%   r_{p_i} - (w \cdot p_i + b) \leq \varepsilon \\
%   (w \cdot p_i + b) - r_{p_i} \leq \varepsilon,
%   \end{aligned}
%   \right.
%   \end{equation}
%   where each equality constraint is approximate with $\varepsilon$ precision. Note that the x-coordinate and y-coordinate are estimated separately.

   Fig. \ref{fig:SVM} shows the empirical CDFs of localization error of the SVM approach with $20\%$ samples for $3$dBm and $10$ dBm noise. We can see that the performance of SVM is quite similar to the kernel approach in Fig. \ref{fig:kernel}. Notice that for adaptive sampling, the allocation ratio $\delta$ does not affect the localization error that much as in the KNN approach and the kernel approach. It seems that for high SNR case, we should allocate more sampling budget to the $1$st-pass sampling, while more sampling budget to the $2$nd-pass sampling for low SNR case. Since for high SNR, the $1$st-pass sampling is able to better locate more informative columns of $\mathcal{G}$ (essentially those more informative columns lies near WiFi access points), while for low SNR it is better to have an accurate estimation of the low-dimensional subspace which is the aim of the $2$nd-pass sampling.

\begin{figure}[t]
\subfigure{\includegraphics[width=0.5\textwidth]{pic/SVM_3dBm.eps}}
\subfigure{\includegraphics[width=0.5\textwidth]{pic/SVM_10dBm.eps}}
\caption{The empirical CDFs for SVM with the same legend as Fig. \ref{fig:KNN}.}\label{fig:SVM}
\end{figure}

\subsubsection{Reduction of Sampled Reference Points}
\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{pic/Budget.eps}
\caption{The sampling budget needed for KNN, kernel approach and SVM.}\label{fig:budget}
\end{figure}

   %From Fig. \ref{fig:KNN}\ref{kernel}\ref{fig:SVM}, we know that tensor completion are the best among existing schemes. Therefore, we are interested in how much sampling budget the proposed adaptive puncturing approach cuts down from from that required by tensor completion. In order to have a fair comparison, we set the localization error for the $95\%$ percentile to be $1$m. Then, we run the recovery-and-localization experiment ten times to calculate the average sampling budget needed. Fig. \ref shows the results for both the high and low SNR cases.

   We are interested in cutting down the sampling budget. We apply the adaptive sampling scheme with $\delta = 1/2$ and then run recovery-and-localization experiment. Through $20$ simulations, keeping these with $[94\% \sim 96\%]$-percentile localization error being $1$m, and calculate the average sampling rate. Fig. \ref{fig:budget} shows the results for both the high and low SNR cases. For high SNR, the kernel approach needs the least sampling budget which is $23\%$, while SVM needs $22\%$ for low SNR. Maintaining similar localization accuracy of KNN, the amount of samples required by the adaptive sampling approach is cut down by $71\% $ for the high SNR case and $55\%$ for the low SNR case.





%\begin{figure}[t]
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/final_40percent_knn.eps}}
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/ft_40percent_knn.eps}}
%\caption{The empirical CDF of localization error and failure rate KNN with $40\%$ samples, $3$dBm noise. TC/T, MC/M, DL/D stands for tensor completion, matrix completion, and direct; $1/2$ and $1/4$ are the case when $\delta = 1/2, 1/4$ and $\gamma = 0.7$.}\label{fig:knn_40percent}
%\end{figure}
%
%\begin{figure}[t]
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/final_40percent_knn_noise.eps}}
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/ft_40percent_knn_noise.eps}}
%\caption{The empirical CDF of localization error and failure rate of KNN with $40\%$ samples, $10$dBm noise.  The same legend with Fig. \ref{fig:knn_40percent}.} \label{fig:knn_40percent_noise}
%\end{figure}

%\begin{figure}[t]
%\centering
%\includegraphics[width=0.65\textwidth]{pic/ft_40percent_knn.eps}
%\caption{The failure rate of KNN localization error with $40\%$ samples. U and P stand for uniform and puncturing; T, M, and D stand for tensor completion, matrix completion, and direct; $1/2$ and $1/4$ are the case when $\delta = 1/2, 1/4$ and $\gamma = 1$.}\label{fig:ft_knn_40percent}
%\end{figure}


%\begin{figure}[t]
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/final_40percent_kernel.eps}}
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/ft_40percent_kernel.eps}}
%\caption{The empirical CDF of localization error and failure rate of Kernel approach with $40\%$ samples, $3$dBm noise. The same legend with Fig. \ref{fig:knn_40percent}.}\label{fig:kernel_40percent}
%\end{figure}
%
%
%\begin{figure}[t]
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/final_40percent_kernel_noise.eps}}
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/ft_40percent_kernel_noise.eps}}
%\caption{The empirical CDF of localization error and failure rate of Kernel approach with $40\%$ samples, $15$dBm noise.  The same legend with Fig. \ref{fig:knn_40percent}.}\label{fig:kernel_40percent_noise}
%\end{figure}
%
%\begin{figure}[t]
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/final_40percent_svm.eps}}
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/ft_40percent_svm.eps}}
%\caption{The empirical CDF of localization error and failure rate of SVM with $40\%$ samples, $3$dBm noise. The same legend with Fig. \ref{fig:knn_40percent}.}\label{fig:svm_40percent}
%\end{figure}
%
%
%\begin{figure}[t]
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/final_40percent_svm_noise.eps}}
%\subfigure{\includegraphics[width=0.5\textwidth]{pic/ft_40percent_svm_noise.eps}}
%\caption{The empirical CDF of localization error and failure rate of SVM with $40\%$ samples, $10$dBm noise.  The same legend with Fig. \ref{fig:knn_40percent}.}\label{fig:svm_40percent_noise}
%\end{figure}

%   In this subsection, we will demonstrate that adaptive puncturing is better than uniform sampling. Also, we show that tensor completion (TC) is better than both matrix completion approach (MC), as well as that without completion (DL, direct).
%
%   Note that from Fig. \ref{fig:recovery}(a) and \ref{fig:recovery}(b), we know that for tensor completion with $40\%$ samples, $\delta = 1/4$ and $\gamma = 0.7$ have recovery errors less than $5\%$. Therefore, we present localization performance of KNN, Kernel approach, and SVM for cases with $40\%$ samples.



 %  Fig. \ref{fig:knn_40percent_noise} shows the empirical CDF of localization error and failure rate of weighted KNN with $40\%$ samples and $10$dBm noise. We can see that as noise level increases, the localization error increases accordingly. The puncturing-enhanced tensor completion has median localization error $0.25$ m, while $90\%$ of test points have localization error less than $1$ m.
%
%   Fig. \ref{fig:kernel_40percent} and Fig. \ref{fig:kernel_40percent_noise} shows the empirical CDFs of localization error and failure rates of Kernel approach with $40\%$ samples, $3$dBm noise and $10$dBm noise. Compared with Fig. \ref{fig:knn_40percent} and Fig. \ref{fig:knn_40percent_noise}, Kernel approach has better localization performance. For $3$dBm noise case, Kernel approach has localization error less than $0.1$ m, while for the $10$dBm case, Kernel approach has failure rate less than $5\%$.
%
%   Fig. \ref{fig:kernel_40percent} and Fig. \ref{fig:kernel_40percent_noise} shows  the empirical CDFs of localization error and failure rates of SVM with $40\%$ samples, $3$dBm noise and $10$dBm noise. Compared with KNN and Kernel approach, SVM relatively better tolerance of noise. Note that the failure rate for $10$dBm case is zero. This shows that our puncturing method can achieve sub-meter indoor localization in low SNR scenarios.
%
%
%

